Non-asymptotic moment bounds for random variables rounded to non-uniformly spaced sets

We study the effects of rounding on the moments of random variables. Specifically, given a random variable $X$ and its rounded counterpart $\operatorname{rd}(X)$, we study $|\mathbb{E}[X^k] - \mathbb{E}[\operatorname{rd}(X)^{k}]|$ for non-negative integer $k$. We consider the case that the rounding function $\operatorname{rd} : \mathbb{R}\to\mathbb{F}$ corresponds either to (i) rounding to the nearest point in some discrete set $\mathbb{F}$ or (ii) rounding randomly to either the nearest larger or smaller point in this same set with probabilities proportional to the distances to these points. In both cases, we show, under reasonable assumptions on the density function of $X$, how to compute a constant $C$ such that $|\mathbb{E}[X^k] - \mathbb{E}[\operatorname{rd}(X)^{k}]| < C\epsilon^2$, provided $|\operatorname{rd}(x) - x| \leq \epsilon \: E(x)$, where $E : \mathbb{R} \to \mathbb{R}_{\geq 0}$ is some fixed positive piecewise linear function. Refined bounds for the absolute moments $\mathbb{E}[ |X^k-\operatorname{rd}(X)^{k}|]$ are also given.

==> tikz_header.tex <==
\usepackage{tikz}
\usetikzlibrary{positioning,decorations.markings,fadings}


\makeatletter
% Code by Mark Wibrow 
% https://tex.stackexchange.com/a/137438/116936
% solution 2
\newif\iftikz@shading@path

\tikzset{
    % There are three circumstances in which the fading sep is needed:
    % 1. Arrows which do not update the bounding box (which is most of them).
    % 2. Line caps/joins and mitres that extend outside the natural bounding 
    %    box of the path (these are not calculated by PGF).
    % 3. Other reasons that haven't been anticipated.
    fading xsep/.store in=\pgfpathfadingxsep,
    fading ysep/.store in=\pgfpathfadingysep,
    fading sep/.style={fading xsep=#1, fading ysep=#1},
    fading sep=0.0cm,
    shading path/.code={%
        % Prevent this stuff happning recursively.
        \iftikz@shading@path%
        \else%
            \tikz@shading@pathtrue%
            % \tikz@addmode installs the `modes' (e.g., fill, draw, shade) 
            % to be applied to the path. It isn't usualy for doing more
            % changes to the path's construction.
            \tikz@addmode{%
                \pgfgetpath\pgf@currentfadingpath%
                % Get the boudning box of the current path size including the fading sep
                \pgfextract@process\pgf@fadingpath@southwest{\pgfpointadd{\pgfqpoint{\pgf@pathminx}{\pgf@pathminy}}%
                    {\pgfpoint{-\pgfpathfadingxsep}{-\pgfpathfadingysep}}}%%
                \pgfextract@process\pgf@fadingpath@northeast{\pgfpointadd{\pgfqpoint{\pgf@pathmaxx}{\pgf@pathmaxy}}%
                    {\pgfpoint{\pgfpathfadingxsep}{\pgfpathfadingysep}}}%
                % Clear the path
                \pgfsetpath\pgfutil@empty%                          
                % Interrupt the path and picture to create a fading.
                \pgfinterruptpath%
                \pgfinterruptpicture%
                    \begin{tikzfadingfrompicture}[name=.]
                        \path [shade=none,fill=none, #1] \pgfextra{%
                            % Set the softpath. Any transformations in #1 will have no effect.
                            % This will *not* update the bounding box...
                            \pgfsetpath\pgf@currentfadingpath%
                            % ...so it is done manually.
                            \pgf@fadingpath@southwest
                            \expandafter\pgf@protocolsizes{\the\pgf@x}{\the\pgf@y}%
                            \pgf@fadingpath@northeast%
                            \expandafter\pgf@protocolsizes{\the\pgf@x}{\the\pgf@y}%
                        };
                        % Now get the bounding of the picture.
                        \xdef\pgf@fadingboundingbox@southwest{\noexpand\pgfqpoint{\the\pgf@picminx}{\the\pgf@picminy}}%
                        \xdef\pgf@fadingboundingbox@northeast{\noexpand\pgfqpoint{\the\pgf@picmaxx}{\the\pgf@picmaxy}}%
                        %
                    \end{tikzfadingfrompicture}%
                \endpgfinterruptpicture%
                \endpgfinterruptpath%
                % Install a rectangle that covers the shaded/faded path picture.                                
                \pgfpathrectanglecorners{\pgf@fadingboundingbox@southwest}{\pgf@fadingboundingbox@northeast}%
                % Make the fading happen.
                \def\tikz@path@fading{.}%
                \tikz@mode@fade@pathtrue%
                \tikz@fade@adjustfalse%10pt
                % Shift the fading to the mid point of the rectangle
                \pgfpointscale{0.5}{\pgfpointadd{\pgf@fadingboundingbox@southwest}{\pgf@fadingboundingbox@northeast}}%
                \edef\tikz@fade@transform{shift={(\the\pgf@x,\the\pgf@y)}}%
            }%
        \fi%
    }
}

\def\MarkLt{3pt}
\def\MarkSep{3pt}

\tikzset{
  TwoMarks/.style={
    postaction={decorate,
      decoration={
        markings,
        mark=at position #1 with
          {
              \begin{scope}[xslant=0.2]
              \draw[line width=\MarkSep,white,-] (0pt,-\MarkLt) -- (0pt,\MarkLt) ;
              \draw[-] (-0.5*\MarkSep,-\MarkLt) -- (-0.5*\MarkSep,\MarkLt) ;
              \draw[-] (0.5*\MarkSep,-\MarkLt) -- (0.5*\MarkSep,\MarkLt) ;
              \end{scope}
          }
       }
    }
  },
  TwoMarks/.default={0.5},
}



